Exploring Multi-Modal Control in Music-Driven Dance Generation

Existing music-driven 3D dance generation methods mainly concentrate on high-quality dance generation, but lack sufficient control during the generation process. To address these issues, we propose a unified framework capable of generating high-quality dance movements and supporting multi-modal control, including genre control, semantic control, and spatial control. First, we decouple the dance generation network from the dance control network, thereby avoiding the degradation in dance quality when adding additional control information. Second, we design specific control strategies for different control information and integrate them into a unified framework. Experimental results show that the proposed dance generation framework outperforms state-of-the-art methods in terms of motion quality and controllability.

==> sections/back/Experiment_dyq.tex <==
\begin{figure}[tbp]
  \centering
  \mbox{} \hfill
  \includegraphics[width=1.0\linewidth]{image/same music different genre.jpg}
  \caption{Generated motions for the same music in different genres, showcasing the effective control of the given genre on the generated sequence and the diversity achieved.
  \label{fig:genre}%
   }
\vspace{-3mm}
\end{figure}

\subsection{Data Processing}
We have chosen the Finedance\cite{FineDance} dataset, which is a music2dance dataset consisting of 22 finely categorized genres, and the currently largest 3D human motion dataset called HumanML3D\cite{humanml3d}, to serve as our cross-modal dataset. We preprocess and unify the motion data into the SMPL\cite{loper2015smpl} format with 22 joints for model training purposes.

\subsection{Implementation Details} 
% 公式里提到的参数记得要写: are set to 1 and 0.5, respectively.
For Motion VQ-VAE, the codebook size is set to $1024 \times 512$. The factor term $\beta$ is 0.02. The downsampling rate $l$ is 4. For both HumanML3D \cite{humanml3d} and Finedance\cite{FineDance} datasets, the motion sequences are concatenated or cropped to $t = 128$ for training. We use AdamW optimizer with [$\beta_1$, $\beta_2$] = [0.9, 0.99], batch size of 128, and exponential moving constant $\lambda$ = 0.99. We train the first $200K$ iterations with a learning rate of 2e-4, and $200K$ with a learning rate of 1e-5. 

For the Cross-modal GPT, we employ 18 transformer\cite{attention} layers with a dimension of 1,024 and 16 heads. The minimum lengths are 40 for both datasets. The maximum length of the music sequence is $T_m$ = 480, and $T_t$ = 100 for the text sequence. The transformer is optimized using AdamW with [$\beta_1$, $\beta_2$] = [0.5, 0.99] and batch size 128. The initialized learning rate is set to 1e-4 for 150K iterations and decayed to 5e-6 for another 800 iterations.
The whole framework {\color{blue}can be trained on a single Tesla V100 GPU.}
%takes about three days on a single 

\begin{figure}[tbp]
  \centering
  \mbox{} \hfill
  \includegraphics[width=1.0\linewidth]{image/same music different motion.jpg}
  \vspace{-9mm}
  \caption{Generated motions for the same music, incorporating different text controls, demonstrate the model's ability to produce movements that correspond to the given textual prompts and can generate fluid routines.
  \label{fig:motion}%
   }
\vspace{-3mm}
\end{figure}

\subsection{Qualitative Results} 
Our model allows for style control, text control, and keyframe control in generating dance motions. Figure \ref{fig:genre} demonstrates the generated movements for the same music segment in different genres. Figure \ref{fig:motion} demonstrates the effects of our model when adding different textual controls to the same music. Figure \ref{fig:duration} demonstrates the different generated results of the same text control under different durations. Figure \ref{fig:keyFrame} illustrates the effectiveness of our model in Key Frame Control. It can be observed that the model can predict a reasonable sequence of actions based on the context, thereby achieving key frame control.

\begin{figure}[tb]
  \centering
  \mbox{} \hfill
  \includegraphics[width=1.0\linewidth]{image/same motion different duration and start time.jpg}
  \caption{Generated motions of the same text control under different durations, further indicating that our model can effectively adapt to different action transitions.
  \label{fig:duration}%
   }
\end{figure}

\begin{figure}[tb]
  \centering
  \mbox{} \hfill
  \includegraphics[width=1.0\linewidth]{image/key frame control.jpg}
  \caption{Key frame control result of our model, {\color{yellow} yellow} parts denotes the key frames and {\color{green} green} parts denotes the mask-predicted motion. The results demonstrate its exceptional capability to accurately predict a cohesive sequence of actions by taking into account the contextual information, thus effectively achieving keyframe control.
  \label{fig:keyFrame}%
   }
\end{figure}


\subsection{Quantitative Comparisons} % mnet

% \begin{table}[ht]
% \caption{Performance Comparison (Part 1 m2d)}
% \label{tab:performance_part1}
% \centering
% \setlength{\tabcolsep}{3.5pt} % 减小列之间的间距
% \begin{tabular}{lccccc}
% \toprule
%     \multirow{2}{*}{\textbf{methods}} & \multicolumn{2}{c}{\textbf{Motion Quality}} & \multicolumn{2}{c}{\textbf{Motion Diversity}}\\
%           & $FID_k$\downarrow & $FID_g$\downarrow & $Div_k$\uparrow & $Div_g$\uparrow & Beat Align\uparrow \\
% \midrule
% Ground Truth & - & - & 10.03 & 7.37 & \\
% \hline
% DanceRevolution\cite{} &  &  &  &  & \\
% DeepDance \cite{} &  &  &  &  & \\
% bailando \cite{} & - & - & - & - & \\
% ours & 36.84 & 59.30 & 8.18 & 12.80 & \\
% \bottomrule
% \end{tabular}
% \end{table}


\begin{table}[ht]
\caption{Performance Comparison (Part 1 m2d)}
\label{tab:performance_m2d}
\centering
\setlength{\tabcolsep}{3.5pt} % 减小列之间的间距
\begin{tabular}{lcccccc}
\toprule
    \multirow{2}{*}{\textbf{methods}} & \multicolumn{2}{c}{\textbf{Motion Quality}} & \multicolumn{2}{c}{\textbf{Motion Diversity}}\\
          & $FID_k$\downarrow & $FID_g$\downarrow & $Div_k$\uparrow & $Div_g$\uparrow \\
\midrule
Ground Truth & - & - & 10.03 & 7.37 \\
\hline
DanceRevolution\cite{dancerevolution} & 380.38 & 412.35 & 15.30 & 5.32 \\
DeepDance \cite{deepdance} & 256.77 & 388.79 & 31.71 & 1.95 \\
Bailando \cite{bailando} & 189.66 & 319.61 & - & - \\
EDGE \cite{edge} & 83.08 & 25.73 & 11.56 & 8.97 \\
FineNet \cite{FineDance}  & - & - & - & - \\ 
Ours & 36.84 & 59.30 & 8.18 & 12.80 \\
Ours & 33.00 & 53.14 & 7.98 & 12.40 \\
\bottomrule
\end{tabular}
\end{table}


\begin{table}[htb]
\caption{User study}
\label{tab:user_study}
\centering
\setlength{\tabcolsep}{2.0pt} % 减小列之间的间距
\begin{tabular}{lcccccc}
\toprule
     \multirow{2}{*}{\textbf{methods}} & \multicolumn{3}{c}{\textbf{Accept Score}} & \multicolumn{3}{c}{\textbf{Control}}\\
     & Quality & Consist & Ctrl & Text & Genre & KF\\
\midrule
DanceRevolution\cite{dancerevolution} & 3.10 & 3.40 & 2.80 &  & \checkmark &  \\
MNET\cite{mnet} & 3.90 & 3.70 & 4.00 &  & \checkmark & \\
Ours(genre) & 3.67 & \textbf{3.78} & 3.75 &  & \checkmark &  \\ % 
\hline
TM2D \cite{tm2d} & 3.50 & 3.60 & 3.70 & \checkmark &  &  \\
Ours(tm2d) & \textbf{3.75} & 3.50 & \textbf{3.70} & \checkmark &  &  \\
\hline
EDGE \cite{edge} & 3.89 & 3.56 & 3.80 &  &  & \checkmark \\
Ours(keyframe) & 3.78 & \textbf{3.67} & 3.67 &  &  & \checkmark \\ % keyframe ctrl
\hline
Ours(overall) & 3.73 & 3.65 & 3.71 & \checkmark & \checkmark & \checkmark \\
\bottomrule
\end{tabular}
\end{table}


We adopt the evaluation settings suggested by Bailando\cite{bailando}  to evaluate the dance generation quality, including FID\cite{fid} and Diversity. As shown in Table \ref{tab:performance_m2d}, our model exhibits significant competitiveness over the baseline in terms of generated results.


% \begin{table}[ht]
% \centering
% % \footnotesize
% % \small % 将表格内容设置为小号字体
% % \tiny % 将表格内容设置为极小号字体
% \caption{Performance Comparison(Part 2 t2d)}
% \label{tab:performance_comparison}
% \setlength{\tabcolsep}{3pt} % 减小列之间的间距
% % \begin{tabular}{p{2.2cm}p{1.5cm}p{1.2cm}p{1.2cm}p{1.5cm}}
% \begin{tabular}{lcccc}
% \toprule
% Methods & R-Precision$\uparrow$ & FID$\downarrow$ & MM Dist$\downarrow$ & Div$\uparrow$ \\
% \hline
% Real motions & 0.511 & 0.002 & 2.974 & 9.503 \\
% \hline
% Seq2Seq \cite{} & 0.180 & 11.75 & 5.529 & 6.223 \\
% Language2Pose \cite{} & 0.246 & 11.02 & 5.296 & 7.676 \\
% Text2Gesture \cite{} & 0.165 & 5.012 & 6.030 & 6.409 \\
% Hier \cite{} & 0.301 & 6.532 & 5.012 & 8.332 \\
% MoCoGAN \cite{} & 0.037 & 94.41 & 9.643 & 0.462 \\
% Dance2Music \cite{} & 0.033 & 66.98 & 8.116 & 0.725 \\
% TM2T \cite{} & 0.424 & 1.501 & 3.467 & 8.589 \\
% T2M-GPT\cite{} & - & - & - & - \\
% Ours & - & - & - & - \\
% \bottomrule
% \end{tabular}
% \end{table}


% \subsection{Ablation studies}
% \label{sec:Ablation}

% \textbf{Window size}
% \label{ablation:windowsize}

% \begin{table}[ht]
% \caption{Ablation Study}
% \label{tab:performance_part1}
% \centering
% \begin{tabular}{lcccc}
% \toprule
%     \multirow{2}{*}{\textbf{Window Size}} & \multicolumn{2}{c}{\textbf{Motion Quality}} & \multicolumn{2}{c}{\textbf{Motion Diversity}}\\
%           & $FID_k$\downarrow & $FID_g$\downarrow & $Div_k$\uparrow & $Div_g$\uparrow\\
% \hline
% 64  & - & - & - & -\\
% 128  & - & - & - & -\\
% 1800 & - & - & - & -\\
% 2000 & - & - & - & -\\
% \bottomrule
% \end{tabular}
% \end{table}

==> sections/back/Intro0905.tex <==
% \section{Introduction}

In today's era of digital entertainment, there is a growing need for the efficient generation of high-quality, controllable 3D dances based on provided music.
With the advancement of technology, the generation of dance sequences that harmonize with music through computer algorithms is becoming a reality.
Most existing works focus on generating high-quality dances that align with the musical genre and rhythm. They strive to reduce artifacts and increase the diversity of generated dances.

%Early research\cite{ofli2011learn2dance, manfre2016automatic, berman2015kinetic} employ motion graph frameworks to synthesis dance from existing dance clips.
%However, these methods are unable to optmize the internal correlations between music and dance clips, and the synthesised dances exhibit a deficiency in diversity.
%There are some methods using deep neural networks for dance generation. Li et al. propose FACT\cite{aist++},
Early methods \cite{aist++,dancerevolution}
input music and seed motions into a Transformer \cite{Transformer} network, generating new dance movements frame by frame in an autoregressive manner, but challenges such as error accumulation and motion frozen phenomena persist.
%With continuous algorithmic advancements,
%Through the persistent efforts of researchers,
%Nowadays,
%There are now methods capable of generating high quality dance sequences based on music.
Recently, some methods can generate high quality dance based on music.
Bailando train a VQ-VAE network to encode dance motion segments into tokens. Subsequently, a Transformer was used to predict dance token sequences from input music, ultimately decoded into 3D dance by a VQ-VAE Decoder. Additionally, Bailando introduce a Actor-Critic  network to enhance the quality of dance actions and mitigate the motion freezing issues present in the FACT network.
FineDance\cite{FineDance} and EDGE\cite{edge} utilize the diffusion\cite{ho2020denoising} model for dance generation, resulting in high-quality and diverse dance sequences. %However, it's important to note that the training process incurs significant computational costs, and the generated outcomes may lack controllability.

However, existing methods have not sufficiently explored the controllability of dance generation.
In practical dance composition, choreographers have the ability to control the genre, semantic, and spatial details of the dance.
Although there are several dance generation methods achieve single-modal control, such as genre control\cite{mnet}, text-based sematic control\cite{tm2d}  and keyframe-based spatial control\cite{edge}, there is still a lack of a unified approch to simultaneously control the genre, semantics, and spatial details of dance.

\begin{figure*}[tbp]
\centering
\mbox{} \hfill
\includegraphics[width=1.0\linewidth]{image/framework-0906-crop.pdf}
\vspace{-8mm}
\caption{Overview of our method. M, T, and G represent Music, Text, and Genre embeddings, respectively.
\label{fig:framework}%
}
\vspace{-3mm}
\end{figure*}

Generating multi-modal controllable dance faces two key challenges: (1) How to ensure both effective control and high-quality dance generation? In previous approaches, dance control and dance generation were tightly coupled, which resulted in a degradation of dance quality when control signals were introduced. This issue becomes more pronounced when multiple modalities of control are simultaneously incorporated.
(2) How to achieve multi-modal control within a unified framework?
%Previous approaches were designed to address single-modal control separately, such as EDGE, which employed diffusion-based mask denoising techniques to achieve keyframes control conveniently.
The genres, text, and keyframes represent three entirely distinct modalities, posing significant challenges to the network's modeling capabilities due to the huge modal gap and the abundance of input signals.

To solve the above issues,
we propose a unified framework for achieving multi-modal controllable and high-quality dance generation.
We decouple dance generation from dance control by pretraining a VQ-VAE. Its encoder can transform dance clips into tokens, and its decoder can reconstruct dances from these tokens. We constrain the control network to predict only these tokens, effectively fixing the VQ-VAE parameters to ensure the quality of generated dance movements. To achieve effective control in the presence of multi-modal input signals, we designed a controllable dance token prediction network based on the GPT architecture. We integrated multi-style embedding networks and multi-genre discriminators to achieve genre control. We also designed a shared latent space for text and music and fused their features for semantic control. Additionally, we utilized GPT's mask predict technique for keyframe control. Our method offers flexibility in achieving controllable dance generation for one or multiple modalities and demonstrates promising results in both qualitative and quantitative experiments.

Our main contributions can be summarized as follows: (1) We propose a unified framework that can generate dance from given music while supporting genre, semantics, as well as the combination control of these modalities.
(2) We decoupled the dance generation network from the dance control network, achieving both effective controllable dance generation and ensuring the quality of the generated dances.

==> sections/back/Introduction_0904.tex <==
% \section{Introduction}

Music and dance, two closely related and time-honored forms of art, have always played a crucial role in various contexts, from celebrations and performances to electronic gaming, animation production, and the presentation of virtual idols. In today's era of digital entertainment, there is a growing and pressing need for the efficient generation of high-quality, controllable 3D dances based on provided music. 

With the advancement of artificial intelligence and computer technology, the generation of dance sequences that harmonize with music through computer algorithms has become a reality.
Most existing works focus on generating high-quality dances that align with the musical genre and rhythm. They strive to reduce artifacts and increase the diversity of generated dances.

%They strive to enhance the coordination between dance and music, aiming for improved dance movement quality.

Early research\cite{ofli2011learn2dance, manfre2016automatic, berman2015kinetic} employed motion graph frameworks for dance synthesis, generating dances by identifying optimal paths within pre-buided motion graphs. In these graphs, each node represented a dance clip, with directed edges reflecting the cost of transitioning between two related motion clips. Essentially, this approach involved resequencing and concatenating existing dance movements to align with the given music. However, the motion graph based methods are unable to learn the internal correlations between music and dance segments, thus unable to synchronize the rhythms of music and dance. Furthermore, the assembled dances, derived by piecing together movements from pre-existing dance database, exhibit a deficiency in diversity.
In recent years, several methods using deep neural networks for dance generation have emerged. Li et al. proposed FACT\cite{aist++}, which input music and seed motions into a Transformer \cite{Transformer} network, generating new dance movements frame by frame in an autoregressive manner.
They have established a new baseline for music-driven dance generation, but challenges such as error accumulation and motion frozen phenomena persist.

With continuous algorithmic advancements, 
%Through the persistent efforts of researchers, 
there are now methods capable of generating high quality dance sequences based on music.
Bailando train a VQ-VAE network to encode dance motion segments into tokens. Subsequently, a Transformer was used to predict dance token sequences from input music, ultimately decoded into 3D dance by a VQ-VAE Decoder. Additionally, Bailando introduce a Actor-Critic  network to enhance the quality of dance actions and mitigate the motion freezing issues present in the FACT network.
FineDance\cite{FineDance} and EDGE\cite{edge} utilize the Diffusion\cite{ho2020denoising} model for dance generation, resulting in high-quality and diverse dance sequences. %However, it's important to note that the training process incurs significant computational costs, and the generated outcomes may lack controllability.

Despite the emergence of numerous endeavors in music-driven dance generation, existing methods have not sufficiently explored the controllability of dance generation. 
In practical dance composition, choreographers have the ability to control the genre, semantic, and spatial details of the dance. There are also several method achieve genre control in dance generation. CycleDance\cite{yin2023dance} is a dance style transfer algorithm devised based on CycleGAN, which can transfer existing dance clips of one dance style into dance clips of another dance style. 
MNET\cite{mnet} propose a multi-genre embedding network and a multi-genre discriminator to achieve genre-controllable dance generation. 
Due to the absence of text-music-dance paired datasets, incorporating semantic control into music-driven dance generation has been a challenging task. 
TM2D train a text encoder and a music encoder respectively, and utilize a shared weight motion decoder to generate dance from both music and text. 
EDGE also achieved spatial control in dance generation by using the standard masked denoising technique of diffusion image inpainting. However, training EDGE comes with a significant computational cost, requiring parallel training on four A100 GPUs.





\begin{figure*}[tbp]
  \centering
  \mbox{} \hfill
  \includegraphics[width=1.0\linewidth]{image/framework - twocol.jpg}
  \vspace{-8mm}
  \caption{Framework
  \label{fig:framework}%
   }
   \vspace{-3mm}
\end{figure*}

As mentioned above, existing music-driven dance algorithms have primarily explored single-modal control and lack a unified method for simultaneously controlling the genre, semantics, and spatial details of the dance.
Generating multi-modal controllable dance faces two key challenges: (1) How to achieve multi-modal control within a unified framework? Previous approaches were designed to address single-modal control separately, such as EDGE, which employed diffusion-based mask denoising techniques to achieve keyframes control conveniently. The genres, text, and keyframes represent three entirely distinct modalities, posing significant challenges to the network's modeling capabilities due to the huge modal gap and the abundance of input signals.
(2) How to ensure both effective control and high-quality dance generation? In previous approaches, dance control and dance generation were tightly coupled, which resulted in a degradation of dance quality when control signals were introduced. This issue becomes more pronounced when multiple modalities of control are simultaneously incorporated.

To solve the above issues,
We propose a unified framework for achieving multi-modal controllable and high-quality dance generation.
We decouple dance generation from dance control by initially pretraining a VQ-VAE. Its encoder can encode dance movements into tokens, and its decoder can reconstruct dances from these tokens. We constrain the control network to predict only these tokens, effectively fixing the VQ-VAE parameters to ensure the quality of generated dance movements. To achieve effective control in the presence of multi-modal input signals, we designed a controllable dance token prediction network based on the GPT architecture. We integrated multi-style embedding networks and multi-genre discriminators to achieve genre control. We also designed a shared latent space for text and music and fused their features for semantic control. Additionally, we utilized GPT's mask predict technique for keyframe control. Our method offers flexibility in achieving controllable dance generation for one or multiple modalities and demonstrates promising results in both qualitative and quantitative experiments.











%Summary

%The fundamental objectives of this study encompass the elevation of music-driven 3D dance generation to new heights through the incorporation of multi-dimensional controllability. Our principal contributions can be delineated as follows:

%Multi-Dimensional Controllability: We present an innovative framework that extends multi-dimensional controllability to dance generation. By enabling precise control over style, semantics, and keyframes, our framework empowers creators to traverse the intricate interplay of artistic expression and computational precision, yielding choreographic masterpieces that resonate with a myriad of creative visions.

%Quantitative and Qualitative Validation: To substantiate the efficiency and robustness of our framework, we meticulously conduct an expansive array of quantitative and qualitative experiments. These experiments not only unveil the strengths and capabilities of our method but also provide an in-depth understanding of its potential to produce visually captivating and conceptually meaningful 3D dance sequences, thus elevating the discourse within the CVPR community.

==> sections/back/Method.tex <==
\textbf{Problem Definition.}
Given the input music, we aim to generate high-quality dance while allowing for control over genre, text, and keyframes simultaneously. 
Given a genre $g$, a text prompt $p$, a piece of motion keyframe $m_k$, and the music feature $y\epsilon\mathbb{R}^{T\times {C_m}}$
%$y = \left\{y_t\right\}_{t=1}^{N}$  
extracted by librosa\cite{librosa}, where $T$ is the feature length and $C_m$ is the feature dimension.
Our method can generate dance
$x\epsilon\mathbb{R}^{T\times {C_t}}$, where $C_t$ is the feature dimension,
%$x=\left\{x_t\right\}_{t=1}^N$ 
corresponding to $y$, while obey the control of $g, p, m_k$. 
The overview of our framework is shown in Fig.~\ref{fig:framework}. 
%Our goals are, first, use $Y$, $g$, and $p$ as a condition and to generate corresponding dance $X=\left\{x_t\right\}_{t=1}^N$, where $\left\{x_t\right\}_{t=i}^j$ is motion corresponding to the text prompt. 
%Second, incorporating $m_k$ to the generated motion and generate coherent dance sequence $X'=\left\{x'_t| x'_k = m_k\right\}_{t=1}^N$, thus enabling key frame control.



\subsection{Motion VQ-VAE}
\label{sec:vqvae}
% 为了保证舞蹈动作的质量，我们将舞蹈生成与控制进行解耦，训练VQ-VAE保证了生成的舞蹈的动作质量。
There is no existing text\&music2dance dataset, but we have $M_m=\left\{x|x\, \text{is music-paired dance}\right\}$ and we also have  $M_t=\left\{x|x\,\text{is text-paired motion}\right\}$. 
We utilize a VQ-VAE to project $M_m \cup M_t$ into a codebook, which is a shared latent space for $M_m$ and $M_t$. By this way, all the motions can be transformed as tokens.
To prevent the degradation in dance quality caused by the addition of control, we decouple dance generation and dance control. We fix the parameters of trained VQ-VAE, and only use the token sequences obtained from the VQ-VAE's encoder to train the dance control network.
%Figure~\ref{fig:framework}. 
%We modified the VQ-VAE in\cite{t2mgpt} to handle our unified data format. The training process is:
%\begin{equation}
%\mathcal{L}_{v q}=\|\hat{M}-M\|_1+\left\|\operatorname{sg}[e]-\hat{e}\right\|_2^2+\beta\left\|e-\operatorname{sg}\left[\hat{e}\right]\right\|_2^2
%\end{equation}
%where $M$ is the ground truth data, $\hat{M}$ is the reconstructed motion, $e$ is the codebook, $\hat{e}$ is the predicted codebook, $sg[\cdot]$ is the stop gradient operation, and $\beta$ is the factor term to adjust the weight of the loss. 

% gpt 部分
\subsection{Cross-modal GPT Framework}
The Cross-modal GPT is a basic model of our dance control network, which is used to achieve music2dance and text2motion respectively. 
\textbf{Text to motion:} We use CLIP\cite{clip} to extract text embedding $T$.
For training text2motion GPT, we follow the \cite{t2mgpt} to maximize the log-likelihood of the data distribution:
\begin{equation} 
\mathcal{L}_{\text {recon }}=\mathbb{E}_{{x} \sim P({M_t})}[-\log p({x} \mid T)]
\end{equation}
where $T$ is the text prompt condition. We perform corrupted sequences for the training-testing discrepancy.
\textbf{Music to dance:} We use MLP  to extract music embedding $M$. The music2dance GPT is trained $\left\{Y, M_m\right\}$, where $Y=\left\{y|y\, \text{is dance-paired music}\right\}$. The training process is similar to text2motion GPT.

As shown in Fig.\ref{fig:framework}, the GPT model consists of Transformer base layer and Transformer head layer, which are primarily composed of linear and attention layers.
To prevent confusion with music and text features, we design two distinct base layers to extract the music/text features respectively. 
We shared the head layer to process the features provided by the base layers and predict the motion tokens. 
%When conducting genre control, the head layer follows the same fusion approach as the M-Base layer. For sequence generation, we utilize Casual self-attention, while for mask prediction, we employ padding self-attention.


%We leverage CLIP\cite{clip} to extract text embedding $T$. 
%To achieve genre control, motivated by existing work\cite{mnet,stargan}, we utilized the mapping network to generate style features $G$ by sampling the latent code $z \sim \mathcal{N}(0, I)$. GPT utilizes known motion to predict the next moment's motion and adds it to the existing motion list. Through an iterative process, a final motion list is obtained.

% 把图片里面相关的结构都介绍一下, 关联性地进行叙述






\subsection{Multi-modal Dance Control Framework}
\subsubsection{Genre Control}
We use the M-Base layer for cross-modal music feature extraction and implementing genre control during the feature extraction stage. 
We employ a mapping network\cite{mnet} to embedding the genre $g$ and random code $\mathbf{z}$ into $G$. The dimension of G is aligned with the music feature $M$. Consequently, we use a cross-attention layer to model the features:
\begin{equation}
\operatorname{CrossAttention}=\operatorname{Softmax}\left(M G^T / \sqrt{d}+B\right) G
\end{equation}
%$Q$, $K$, and $V$ are the query, key, and value metrics, 
where $B$ is the bias, $d$ is a scaling factor to ensure the stability of the model's training process.

We use MLP for the extraction of music feature $M$ to ensure that the feature dimension is consistent with $T$ and feed the music features into GPT sequentially. 
For training music2dance with genre control, we adopt the training strategy\cite{mnet}:
\begin{equation}
\begin{aligned}
\mathcal{L}_{\text {genre }}= & \mathbb{E}_{x \sim P_{M_m}}\left[\log D\left(x, g, y\right)\right]+ \\
& \mathbb{E}_{\mathbf{z} \sim \mathcal{N}(0, \mathbf{I})}\left[\log \left(1-D\left(GPT\left(\mathbf{z}, g, y\right), g, y\right)\right)\right],
\end{aligned}
\end{equation}
where the $D(\cdot)$ is the multi-genre dance discriminator.
% to assessing the dance sequence from the real ones corresponding to the specific genre $g$, $z$ is the random code. %We replaced the origin\cite{mnet} reconstruction loss with the maximization of the log-likelihood. 



\subsubsection{Music-genre-text Fusion}
\label{sec:fusion}
% 在规定了融合区间后，我们在前10%和后10%的区间进行特征权重相加。 在某一个融合区间内，我们同时使用 Base-M 和 Base-T 进行特征提取，并按照 Base-T 的特征长度长度截取Base-M 的相应部分进行 fusion。fusion 得到的特征将被放入 head, 从而得到下一个时刻的 motion token.

Thanks to the VQ-VAE we've trained on $\left\{M_m, M_t\right\}$, capable of decoding semantically meaningful motions; and the text2motion GPT model we've developed, trained on $\left\{M_t, p\right\}$, excels at extracting text features and predicting motion tokens.
We are able to introduce semantic control into our dance generation process. However, directly incorporating semantic movements into the dance can significantly deteriorate the quality of the dance, resulting in severe incoherence. 
Therefore, we set a transitional interval in which where we fusion music features $M$ extracted from the M-base and text features $T$ extracted from the T-base, formulated as:
\begin{equation}
F_i=T_i*(1-w_i)+M_i*w_i
\end{equation}
where $F_i$ is the fusion feature and $w_i$ is the fusion weight. The weight change pattern provided by Fig.\ref{fig:fusion}.
Subsequently, the fused feature $F_i$ is inputted to the head layer to predict the dance tokens with the guidance of text. Finally, using the pre-trained VQ-VAE decoder can reconstruct the 3D dance from tokens.
%After specifying the fusion intervals, we perform feature weight summation within the first 10\% and last 10\% intervals. As shown in Figure \ref{fig:fusion}, the T-Base layer and M-Base layer simultaneously perform feature extraction on the generated tokens. At time step $i$, the extracted features are $T_i$ and $M_i$, respectively. These features are then weighted and combined according to the weight change pattern provided in Figure \ref{fig:fusion}. 

\label{sec:gpt}
    % fig
\begin{figure}[tbp]
  \centering
  \mbox{} \hfill
  \includegraphics[width=1.0\linewidth]{image/Fusion-0907.pdf}
  \vspace{-8mm}
  \caption{{Text control module.}
  \vspace{-3mm}
  \label{fig:fusion}%
   }
\end{figure}

\subsubsection{Key Frame Control}
\label{sec:Frame control}
Based on the GPT framework, we employ the mask and predict mechanism to achieve keyframe control. First, we use the GPT model (with Casual Attention Layer) to generate dance tokens based on the music. Subsequently, we encode the keyframes that need to be controlled into tokens and insert them into the previously generated token sequence. We mask out the keyframes to enable GPT  (with Mask Attention Layer) to predict the before and after k motion tokens, thereby achieving keyframe control while ensuring the coherence of the generated dance sequence. 
By modifying the attention layer of causal attention or mask attention, different functions such as sequence generation and keyframe control can be achieved.
%Similar to NLP processing, utilizing the GPT framework makes is convenient to perform sequence mask prediction, thus achieving keyframe control. Based on the dance token sequence generated by the aforementioned GPT, we insert keyframe tokens and mask $k$ motion tokens before and after the keyframe tokens, and then perform mask prediction. By replacing the attention layer of the head with padding self-attention and retraining, keyframe control of dance movements can be achieved. 

\begin{equation}
\operatorname{MaskAttention}=\operatorname{Softmax}\left(Q K^T / \sqrt{d}+B\right) \times mask 
\end{equation}
Where mask is set to 1 at keyframe positions and to 0 at positions where predictions are needed.

==> sections/back/Method_dqy.tex <==
\textbf{Problem Definition.}
Given the input music, we aim to generate high-quality dance while allowing for control over genre, text, and keyframes simultaneously. 
Formally, given a genre $g$, a text prompt $p$, a piece of motion keyframe $m_k$, and a clip of music $Y = \left\{y_t\right\}_{t=1}^{N}$ where $N$ is the music length, our goals are, first, use $Y$, $g$, and $p$ as a condition and to generate corresponding dance $X=\left\{x_t\right\}_{t=1}^N$, where $\left\{x_t\right\}_{t=i}^j$ is motion corresponding to the text prompt. Second, incorporating $m_k$ to the generated motion and generate coherent dance sequence $X'=\left\{x'_t| x'_k = m_k\right\}_{t=1}^N$, thus enabling key frame control.
The overview of our framework is shown in Figure~\ref{fig:framework}. 

\subsection{Motion VQ-VAE}
\label{sec:vqvae}
% 为了保证舞蹈动作的质量，我们将舞蹈生成与控制进行解耦，训练VQ-VAE保证了生成的舞蹈的动作质量。
Since there is no existing text\&music2dance dataset, we utilize a VQ-VAE to project the motions into a consistent and shared latent space, which is represented with a codebook, which enabling semantic alignment of the datasets. The framework is illustrated in Figure~\ref{fig:framework}. 
We modified the VQ-VAE in\cite{t2mgpt} to handle our unified data format. The training process is:
\begin{equation}
\mathcal{L}_{v q}=\|\hat{M}-M\|_1+\left\|\operatorname{sg}[e]-\hat{e}\right\|_2^2+\beta\left\|e-\operatorname{sg}\left[\hat{e}\right]\right\|_2^2
\end{equation}
where $M$ is the motion data, $\hat{M}$ is the reconstructed motion, $e$ is the codebook, $\hat{e}$ is the predicted codebook, $sg[\cdot]$ is the stop gradient operation, and $\beta$ is the factor term to adjust the weight of the loss. 

% gpt 部分
\subsection{Cross-modal GPT Framework}
Our Cross-modal GPT architecture is illustrated in figure \ref{fig:framework}, where we share the head layer and utilize two distinct base layer to accomplish the tasks of music\&genre2dance and text2motion simultaneously. We leverage CLIP\cite{clip} to extract text embedding $T$. To achieve genre control, motivated by existing work\cite{mnet,stargan}, we utilized the mapping network to generate style features $G$ by sampling the latent code $z \sim \mathcal{N}(0, I)$. GPT utilizes known motion to predict the next moment's motion and adds it to the existing motion list. Through an iterative process, a final motion list is obtained.

% 把图片里面相关的结构都介绍一下, 关联性地进行叙述
\textbf{Text Transformer Base Layer(T-Base):} 
Adopted from\cite{t2mgpt}, we use T-Base {\color{blue}layer} for cross-modal feature extraction of $T$ and motion feature to prevent confusion with dance motion features extracted from M-Base layer and enhance specificity.

\textbf{Music Transformer Base Layer(M-Base):}
Based on the structure of Base-T, Base-M achieves feature fusion of dance motion and genre through self-attention:
\begin{equation}
\operatorname{Attention}=\operatorname{Softmax}\left(Q K^T / \sqrt{d}+B\right) V
\end{equation}
Where $Q$, $K$, and $V$ are the query, key, and value metrics, $B$ is the bias. Here we let the motion feature be $Q$, the genre feature be $K$, and $V$.

\textbf{Transformer Head Layer(Head):}
Inspired by\cite{t2mgpt}, we utilize the head layer to process the features provided by the base layers and obtain the motion prediction. When conducting genre control, the head layer follows the same fusion approach as the M-Base layer. For sequence generation, we utilize Casual self-attention, while for mask prediction, we employ padding self-attention.

\subsection{Text to Motion}
To extract semantic information of motion from text, it is necessary to train a T-Base layer for text2motion feature extraction, as well as a shared weight Head for motion prediction.
For training text2motion, we follow the \cite{t2mgpt} to maximize the log-likelihood of the data distribution：
\begin{equation} 
\mathcal{L}_{\text {recon }}=\mathbb{E}_{X \sim p(X)}[-\log p(X \mid c_p)]
\end{equation}
Where $c_p$ is the text prompt condition. We perform corrupted sequences for the training-testing discrepancy.

\subsection{Music \& Genre to Dance}
We use M-Base {\color{blue}layer} for cross-modal music feature extraction and implementing genre control during the feature extraction stage. 
We use MLP for the extraction of music feature $M$ to ensure that the feature dimension is consistent with $T$ and feed the music features into GPT sequentially. 
For training music2dance with genre control, we adopt the training strategy\cite{mnet}:
\begin{equation}
\begin{aligned}
\mathcal{L}_{\text {genre }}= & \mathbb{E}\left[\log D\left(\mathbf{X}, g, \mathbf{Y}\right)\right]+ \\
& \mathbb{E}_{\mathbf{z}}\left[\log \left(1-D\left(GPT\left(\mathbf{X}, g, \mathbf{Y}\right), g, \mathbf{Y}\right)\right)\right],
\end{aligned}
\end{equation}
where the $D_g(\cdot)$ is the discriminator to distinguish the dance sequence from the real ones corresponding to the specific genre $g$, $z \in \mathcal{Z}$ is the latent code. We replaced the origin\cite{mnet} reconstruction loss with the maximization of the log-likelihood. 



\subsection{Music-genre-text Fusion}
\label{sec:fusion}
% 在规定了融合区间后，我们在前10%和后10%的区间进行特征权重相加。 在某一个融合区间内，我们同时使用 Base-M 和 Base-T 进行特征提取，并按照 Base-T 的特征长度长度截取Base-M 的相应部分进行 fusion。fusion 得到的特征将被放入 head, 从而得到下一个时刻的 motion token.
After specifying the fusion intervals, we perform feature weight summation within the first 10\% and last 10\% intervals. As shown in Figure \ref{fig:fusion}, the T-Base layer and M-Base layer simultaneously perform feature extraction on the generated tokens. At time step $i$, the extracted features are $T_i$ and $M_i$, respectively. These features are then weighted and combined according to the weight change pattern provided in Figure \ref{fig:fusion}. Subsequently, the fused feature is inputted to the head layer to obtain the next time step's action prediction.

\label{sec:gpt}
    % fig
\begin{figure}[tbp]
  \centering
  \mbox{} \hfill
  \includegraphics[width=1.0\linewidth]{image/Fusion.jpg}
  \caption{{\color{blue}Text control module}
  \label{fig:fusion}%
   }
\end{figure}

\subsection{Key Frame Control}
\label{sec:Frame control}
Similar to NLP processing, utilizing the GPT framework makes it convenient to perform sequence mask prediction, thus achieving keyframe control. Based on the motion sequence generated by the aforementioned GPT, we insert keyframes and then mask the motion tokens before and after the keyframes, and then perform mask prediction. By replacing the attention layer of the head with padding self-attention and retraining, keyframe control of dance movements can be achieved. By modifying the masking strategy of attention in the head layer, different functions such as sequence generation and keyframe control can be achieved:
\begin{equation}
\operatorname{MaskAttention}=\operatorname{Softmax}\left(Q K^T / \sqrt{d}+B\right) \times mask 
\end{equation}}
